The Engagement-Prolonging Designs Teens Encounter on Very Large Online Platforms

In the attention economy, online platforms are incentivized to design products that maximize user engagement, even when such practices conflict with users' best interests. We conducted a structured content analysis of all Very Large Online Platforms (VLOPs) to identify the designs these influential apps and sites use to capture attention and extend engagement. Specifically, we conducted this analysis posing as a teenager to identify the designs that young people are exposed to. We find that VLOPs use four strategies to extend teens' use: pressuring, enticing, trapping, and lulling them into spending more time online. We report on a hierarchical taxonomy organizing the 63 designs that fall under these categories. Applying this taxonomy to all 17 VLOPs, we identify 583 instances of engagement-prolonging designs, with social media platforms using twice as many as other VLOPs. We present three vignettes illustrating how these designs reinforce one another in practice. We further contribute a graphical dataset of videos illustrating these features in the wild.

==> mainacm.tex <==
\newcommand{\remove}[1]{{\color{red} \sout{#1}}}
%\newcommand{\change}[1]{{\color{blue} \uwave{#1}}}
\newcommand{\change}[1]{{\color{blue} #1}}


==> sections/scratch.tex <==
% Table 1: Manipulative Designs that Target Users’ Attention as Distilled by Monge Roffarello et al. 
% Pattern Name
% Main Context of Use
% P1 - Infinite Scroll
% Social media
% P2 - Casino Pull-to-refresh
% Social media on smartphones
% P3 - Neverending Autoplay
% Social media and video streaming
% P4 - Guilty Pleasure Recommendations
% Social media and video streaming
% P5 - Disguised Ads and Recommendations
% Social media
% P6 - Recapture Notifications
% Social media, video streaming, messaging 
% P7 - Playing by Appointment
% Video games and social media
% P8 - Grinding
% Video games and social media
% P9 - Attentional Roach Motel
% Social media
% P10 - Time Fog
% Video streaming platforms
% P11 - Fake Social Notifications
% Video games and social media
